Data complexity of answering conjunctive queries over SHIQ knowledge bases

An algorithm for answering conjunctive queries over SHIQ knowledge bases that is coNP in data complexity is given. The algorithm is based on the tableau algorithm for reasoning with individuals in SHIQ. The blocking conditions of the tableau are weakened in such a way that the set of models the modified algorithm yields suffices to check query entailment. The modified blocking conditions are based on the ones proposed by Levy and Rousset for reasoning with Horn Rules in the description logic ALCNR.

==> conjQuerNoTrans.tex <==
\section{Answering Conjunctive Queries}

\begin{definition}[conjunctive query]
A \emph{conjunctive query} over a knowledge base $K$ is a sentence of the form 
	\begin{displaymath}
		(\exists \vect{Y}).p_1(\ol{Y_1})\ld{\land}p_n(\ol{Y_n})
	\end{displaymath}
where $p_1 \cld p_n$ are either roles in $\roles{K}$ or concepts in $\C_{K}$;
$\vect{Y_1} \cld \vect{Y_n}$ are tuples of variables and constants
and $\vect{Y} \subseteq \vect{Y_1} \ld{\cup} \vect{Y_n}$. 
The variables in $Q$ are denoted by $V_Q =  \vect{Y_1} \ld{\cup} \vect{Y_n}$. 
The set of literals in $Q$ is $L_Q = \set{p_1(\ol{Y_1}) \cld p_n(\ol{Y_n})}$, and the cardinality of $L_Q$ will be denoted by $n_Q$.
\end{definition}

Conjunctive queries are interpreted as in standard first order logic, i.e. $\I = \inter{I}$ is a model of $Q$ if there is a mapping $\sigma$ from the variables in $Q$ to objects in $\dom{I}$ such that $\sigma(\vect{Y}) \in \Int{I}{p}$ for all $p(\vect{Y}) \in L_Q$.
For a knowledge base $K$ and a query $Q$, we say that $K \models Q$ iff for every interpretation $\I$, $\I \models K$ implies $\I \models Q$.
Analogously, for a completion forest $\F$ and a query $Q$, we say that $\F \models Q$ iff for every interpretation $\I$, $\I \models \F$ implies $\I \models Q$.

\begin{definition}[Conjunctive Query Entailment]
Let $K$ be a knowledge base and let $Q$ be cojunctive query. 
The \emph{conjunctive query entailment} problem is to decide whether $K \models Q$. 
\end{definition}

In the following sections, we will use $Q$ to denote a conjunctive query.
We say that a completion forest $\F$ entails a query $Q$, denoted $\models_{\F} Q$, 
if there is a mapping $\sigma:V_Q \ra V_{\F}$ such that 
    \begin{enumerate}
	\item\label{cond1map}
	For all $C(x) \in L_Q$, $C \in \labelfunc{\sigma(x)}$.
	\item\label{cond2map}
	For all $R(x,y) \in L_Q$, there is some $S \SUBSTRANS R$ such that either 
		$S \in \labelfunc{\tup{\sigma(x),\sigma(y)}}$  or
		$S \in \mathbf{R}_{+}$ and $\sigma(y)$ is an $S$-descendant of $\sigma(x)$.
    \end{enumerate}

\begin{lemma} \label{lemmaifforestthenallmodels}
If $\models_{\F} Q$, then $\F \models Q$.
\end{lemma}

\begin{proof}
Since $\models_{\F} Q$, 
there is a mapping $\sigma:V_Q \ra V_{\F}$ satisfying conditions~\ref{cond1map} and ~\ref{cond2map}.
Take any arbitrary model $\I = \inter{I}$ of $\F$. By definition, it satisifies the following:
    \begin{itemize}
	\item
	if $C \in \labelfunc{x}$, then $\Int{I}{x} \in \Int{I}{C}$
	\item
	if $S \in \labelfunc{\tup{x,y}}$ and $S \SUBSTRANS R$, then $\tup{\Int{I}{x}, \Int{I}{y}} \in \Int{I}{R}$.
	\item
	if $\sigma(y)$ is an $S$-descendant of $\sigma(x)$, $S \in \mathbf{R}_{+}$ and $S \SUBSTRANS R$, then $\tup{\Int{I}{x}, \Int{I}{y}} \in \Int{I}{R}$.
	\item
	if $x \NEQ y \in \F$, then  $\Int{I}{x} \neq  \Int{I}{y}$
    \end{itemize}  

We can define a mapping $\phi$ from the variables in $V_Q$  to objects in $\dom{I}$ as $\phi(x) = \Int{I}{\sigma(x)}$, and this mapping satisfies $\phi(\vect{Y}) \in \Int{I}{p}$ for all $p(\vect{Y}) \in L_Q$.
\end{proof}

We will prove that if a query is entailed by the canonical interpretation of the tableau induced by a forest, then it is entailed by the forest itself. 
For this purpose, we will show that if there is a way to map the variables of the query to variables in the induced tableau, equiv. to paths in the forest, then the query variables can be mapped to the nodes in the forest in such a way that any model of the forest will also be a model of the query.

\begin{proposition}\label{canonicalmodelsQ}

Consider $\F \in \mathsf{ccf}(\nforests{F}{K}{n_Q})$, and 
let $\I_{\F}$ be the canonical model of the tableau induced by $\F$. 
If $\I_{\F} \models Q$ then $\models_{\F} Q$.
\end{proposition}

\begin{proof}
Since $\I_{\F} \models Q$, then there is a mapping $\sigma:V_Q \ra V_{T_{\F}}$ s.t.
\begin{itemize}
\item
For all $C(x) \in L_Q$, $C \in \tab{L}(\sigma(x))$.
\item 
For all $R(x,y) \in L_Q$, $\tup{\sigma(x),\sigma(y)} \in \valclos{\tab{E}(R)}$.
\end{itemize}

By definition, $\tup{\sigma(x),\sigma(y)} \in \valclos{\tab{E}(R)}$ implies that 
$\tup{\sigma(x),\sigma(y)} \in \tab{E}(S)$ for some $S \SUBSTRANS R$ or 
$\tup{\sigma(x),\sigma(y)} \in \tab{E}(S)^{+}$ for some $S \SUBSTRANS R$, $S \in \mathbf{R}_{+}$.

We will define a new mapping $\sigma':V_Q \ra V_{\F}$. 
We define the set of variables in $V_Q$ that are mapped by $\sigma$ to a path that has a subpath ending in a leaf of a blocked $n$-tree: 
\begin{displaymath}
\ssfunc{afterblocked}{V_Q} = \set{x \in V_Q \st \text{for some $p$  subpath of $\sigma(x)$, } \tail{p} \neq  \tailp{p}}
\end{displaymath}
Note that if $\ssfunc{afterblocked}{V_Q} \neq \emptyset$, all variables in $V_Q \setminus \ssfunc{afterblocked}{V_Q}$ are tree blocked. In this case, let $\psi$ denote the isomorphism between the variables in $V_Q \setminus \ssfunc{afterblocked}{V_Q}$ and the variables that tree-block them. 
Otherwise, let $\psi$ be the identity function.
The mapping $\sigma':V_Q \ra V_{\F}$ is defined as follows:

    \begin{displaymath}
	\sigma'(x)  = \left\{\
	\begin{array}{ll}
		\tailp{\sigma(x)}       & \text{  if } x \in \ssfunc{afterblocked}{V_Q}\\
		\psi(\tailp{\sigma(x)}) & \text{  otherwise}
	\end{array}
	\right .
    \end{displaymath}

Now we will show that the mapping $\sigma'$ has the following properties:
\begin{enumerate}
\item\label{conc}
If $C \in \tab{L}(\sigma(x))$, then $C(x) \in L_Q$, $C \in \L((\sigma'(x)))$.
\item\label{role} 
If $\tup{\sigma(x),\sigma(y)} \in \tab{E}(S)$, then $S \in \L(\tup{\sigma'(x),\sigma'(y)})$.
\item\label{roleT} 
If $\tup{\sigma(x),\sigma(y)} \in \tab{E}(S)^{+}$, then $\sigma'(y)$ is an $S$-descendant of $\sigma'(x)$.
\end{enumerate}

The proof of~\ref{conc} is trivial, since $\tab{L}(\sigma(x)) =  \labelfunc{\tail{\sigma(x)}} =  \labelfunc{\psi(\tail{\sigma(x)})}$, 
so $\tab{L}(\sigma(x)) = \labelfunc{\sigma'(x)}$.\\
To prove~\ref{role}, we will prove that if $\tup{\sigma(x),\sigma(y)} \in \tab{E}(S)$, then $\sigma'(x)$ is an $S$-neighbour of $\sigma'(y)$.
Let $u = \sigma(x)$ and $v = \sigma(y)$.
By definition, if $\tup{u,v} \in \tab{E}(S)$, 
then we have one of the following cases:
\begin{enumerate}[{\it i)}]
    \item
	$u = \path{\pn{a_i}{a_i}}$ and $v = \path{\pn{a_j}{a_j}}$ for some root nodes 
	$a_i$, $a_j$ in $\F$ s.t. $a_i$ is an $S$-neighbour of $a_j$.
	Since $\sigma'(x) = \tailp{u} = a_i$ is an $S$-neighbour of 
	$\sigma'(y) = \tailp{v} = a_j$, the claim holds. 
	\\
    \item \label{succitem}
	$v$ is an $S$-step of $u$, i.e. 
	$v = \path{u \st \pn{z}{z'}}$ for some $z'$ $S$-successor of $\tail{u}$.
	We will consider some subcases. 	
	Note that since $v$ is an $S$-step of $u$, it can not be the case that $x$ is in $\ssfunc{afterblocked}{V_Q}$ and $y$ is not. 
	\begin{enumerate}[(a)]
	    \item
		Both $x$ and $y$ are in $\ssfunc{afterblocked}{V_Q}$.\\
		In this case we have that $\tailp{v} = z = z'$ 
		and $\tailp{u} = \tail{u}$. Since 
		$\sigma'(x) = \tail{u}$ and 
		$\sigma'(y) = z'$,
		we get $\sigma'(y)$ is an $S$-successor of $\sigma'(x)$ as desired.
	    \item
		Neither $x$ nor $y$ are in $\ssfunc{afterblocked}{V_Q}$.\\ 		
		Note that in this case $u$ can not finish in a leaf node, so
		$\tail{u} = \tailp{u}$.
		By definition, $\sigma'(x) = \psi(\tailp{u})$ and 
		$\sigma'(y) = \psi(\tailp{v}) = \psi(z')$.
		Since  $z'$ is an $S$-successor of $\tail{u}$, 
		then  $z'$  is an $S$-successor of $\tailp{u}$
		and hence  $\psi(z')$ $S$-successor of $\psi(\tailp{u})$, so
		$\sigma'(y)$ is an $S$-successor of $\sigma'(x)$ as desired.
	    \item
		$x$ is not in  $\ssfunc{afterblocked}{V_Q}$, but $y$ is.\\
		In this case we have that $u$ ends in a leaf node and $\tail{u} = \psi(\tailp{u})$.
		By definition, $\sigma'(x) = \psi(\tailp{u}) = \tail{u}$ and 
		$\sigma'(y) = \tailp{v} = z'$, so
		$\sigma'(y)$ is again an $S$-successor of $\sigma'(x)$.
	\end{enumerate}
    \item
	$u$ is an $\inverse{S}$-step of $u$, i.e. 
 	$v = \path{u \st \pn{z}{z'}}$ for some $z'$ $\inverse{S}$-successor of $\tail{u}$.
	Analogous to case~{\it\ref{succitem})}, we prove that $\sigma'(y)$ is an $\inverse{S}$-successor of $\sigma'(x)$ in all cases. Thus it is also the case that $\sigma'(x)$ is an $S$-neighbour of $\sigma'(y)$ and the claim holds. 
\end{enumerate}

Since the mapping $\sigma'$ has properties \ref{conc} and \ref{role}, $\models_{\F} Q$.
\end{proof}

\begin{proposition}\label{legalforstsQ}
$K \models Q$ iff $\F \models Q$ for every $\F \in \mathsf{ccf}(\nforests{F}{K}{n_Q})$.
\end{proposition}

\begin{proof}
The only if direction is trivial. 
Consider any $\F \in \nforests{F}{K}{n_Q}$. 
Since any model $\I$ of $\F$ is a model of $K$ (Remark~\ref{FmodelsK})
then $K \models Q$ implies $\F \models Q$.
The if direction can be done by contraposition. 
If $K \nvDash Q$, then there is some model $\I$ of $K$ such that $\I \nvDash Q$. 
By Propostion~\ref{KmodelssomeF}, $\I \models \F$ for some $\F \in \mathsf{ccf}(\nforests{F}{K}{n_Q})$, 
and we have that $\F  \nvDash Q$ for some $\F \in \mathsf{ccf}(\nforests{F}{K}{n_Q})$.
\end{proof}

The following theorem states the correctness of the algorithm: to solve the entailment problem of a query it suffices to check wheter it is entailed by each of the complete and crash free completion forests of the knowledge base. 

\begin{theorem}\label{kiffallcompf}
$K \models Q$ iff $\models_{\F} Q$ for every $\F \in \mathsf{ccf}(\nforests{F}{K}{n_Q})$.
\end{theorem}

\begin{proof}
First we prove that if $K \models Q$ then $\models_{\F} Q$.
Take any arbitrary $\F \in \mathsf{ccf}(\nforests{F}{K}{n_Q})$. 
Since $K \models Q$,  then  $\F \models Q$ (Propostition~\ref{legalforstsQ}). 
In particular, we have that $\I_{\F} \models Q$, where $\I_{\F}$ is the canonical model of the tableau induced by $\F$.
Thus, by Proposition~\ref{canonicalmodelsQ}, $\models_{\F} Q$.

To prove the other direction, observe that  from $\models_{\F} Q$ and Lemma~\ref{lemmaifforestthenallmodels}, 
we have that $\F \models Q$ for every $\F \in \mathsf{ccf}(\nforests{F}{K}{n_Q})$.
Finally, by  Propostition~\ref{legalforstsQ}, $K \models Q$.
\end{proof}





==> constSys.tex <==
\subsection{An  Constraint System for a Knowledge Base} 

A constraint system is only an alternative notation of an A-Box and a T-Box. 
It contains all assertions of the A-Box, as well as statments of the form $\forall x.C(x)$ as given in~\cite{levy00} to represent concept inclusion axioms and the \emph{choose-rule}. 
The equality and inequlity predicates are used to allow/disallow non-unique names of objects.

If not stated otherwise, in the following 
$K$ will denote a $\dlf{SHIQ}$ knowledge base $K = \tup{\krbox{A},\krbox{R},\krbox{T}}$,
$\roles{A,T}$ the roles occurring in $\krbox{A} \cup \krbox{T} \cup \krbox{R}$ together wih their inverses
and $\indivs{A}$ the individual names occurring in $\krbox{A}$.

\begin{definition}[Constraint System]
Let $C$ denote a concept;
$R$ a role,
$a,b$ individuals and 
$x$ a variable.
A constraint system $S$ is a set of statements of the form:
$C(a)$, 
$R(a,b)$, 
$\forall x.C(x)$,
$s = t$,
$s \neq t$.
The set $\axioms{S} := \set{C \st \forall x.C(x) \in S}$ will denote the \emph{axioms} of $S$.
\end{definition}

\begin{definition}[Constraint System for $\krbox{A}, \krbox{T}$]
Given a $\dlf{SHIQ}$ A-Box $\krbox{A}$ and a T-Box $\krbox{T}$, a constraint system $S_{\krbox{A},\krbox{T}}$ for $\krbox{A} \cup \krbox{T}$ 
is (the smallest) constraint system satisfying the following:
\begin{enumerate}
\item
Every assertion in $\krbox{A}$ is in $S$.
\item
For every concept inclusion axiom $C \SUBS D$ in $\krbox{T}$,  
$\forall x.\NOT C \OR D(x)$ is in $S$.
\item
For every concept name $C$ ocurring in $\clos{A}$ ($\cup \clos{T}$?),  
$\forall x.C \OR \NOT C(x)$ is in $S$.
\item
For every pair of individual names $a,b$ ocurring in in $\krbox{A}$,  
$a \neq b$ is in $S$.
\end{enumerate}
\end{definition}

\begin{remark}
Any model of a constraint system $S_{\krbox{A}, \krbox{T}}$ is also a model of
$\krbox{A} \cup \krbox{T}$.
\end{remark}

